On the Strength of Character Language Models for Multilingual Named Entity Recognition

Character-level patterns have been widely used as features in English Named Entity Recognition (NER) systems. However, to date there has been no direct investigation of the inherent differences between name and non-name tokens in text, nor whether this property holds across multiple languages. This paper analyzes the capabilities of corpus-agnostic Character-level Language Models (CLMs) in the binary task of distinguishing name tokens from non-name tokens. We demonstrate that CLMs provide a simple and powerful model for capturing these differences, identifying named entity tokens in a diverse set of languages at close to the performance of full NER systems. Moreover, by adding very simple CLM-based features we can significantly improve the performance of an off-the-shelf NER system for multiple languages.

==> excised.tex <==
% \begin{table*}[!ht]
% \centering
% \begin{tabular}{lrrrrrr}
% \toprule
% \multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{CAP}} & \multirow{2}{*}{\textbf{NEI}} & \multicolumn{4}{c}{\bf NER}\\ 
%  & & & \textbf{PER} & \textbf{LOC} & \textbf{ORG} & \textbf{Overall}\\ 
%  \midrule
% \textbf{English} & 83.8 & 87.2 & & &  & \\ 
% \textbf{Uzbek} && 80.1 &  & & & 57.3 \\ 
% \textbf{Amharic} & - & 71.6 &  & & & 44.4 \\ 
% \textbf{Tamil} & - & 69.1 &  & & & 51.6 \\ 
% \textbf{Arabic} & - & 58.6 & & &  & 27.9 \\ 
% \textbf{Hausa} &  & 67.4 &  &  &  & 45.4 \\ \bottomrule
% \end{tabular}
% \caption{
% {\bf Performance of Character-level Language Models on NEI and NER tagging when trained with labeled data.}
% 'CAP' is the Capitalization-only baseline. 'NEI' is the Named Entity Identification task, which finds only spans, no labels. 'NER' results are phrase-level F1 scores; All scores are F1 scores. 
% } % end caption
% \label{tab:neGold}
% \end{table*}

% \begin{table*}[!ht]
% \centering
% \begin{tabular}{lrrrrrr}
% \hline
% \multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{CAP}} & \multirow{2}{*}{\textbf{NEI}} & \multicolumn{4}{c}{\bf NER}\\ 
%  & & & \textbf{PER} & \textbf{LOC} & \textbf{ORG} & \textbf{Overall}\\ \hline
% \textbf{English} &  &  & & &  & \\ 
% \textbf{Uzbek} &&  &  & & & 41.3 \\ 
% \textbf{Amharic} & - &  &  & & & 43.4 \\ 
% \textbf{Tamil} & - &  &  & & & 20.6 \\ 
% \textbf{Arabic} & - &  & & &  & 21.4 \\ 
% \textbf{Hausa} &  &  &  &  &  & 43.5 \\ \bottomrule
% \end{tabular}
% \caption{
% {\bf Performance of Character-level Language Models on NEI and NER tagging when trained with found data.}
% 'CAP' is the Capitalization-only baseline. 'NEI' is the binary Named Entity Recognition task. 'NER' results are token-level F1 scores; 'Overall' is the \ms{micro? macro?} average of the class F1 scores. 
% } % end caption
% \label{tab:neFound}
% \end{table*}


% \begin{table*}[!ht]
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Language}} & \multicolumn{4}{|c|}{\bf NER}\\ 
%   & \textbf{PER} & \textbf{LOC} & \textbf{ORG} & \textbf{Overall}\\ \hline
% $ \textbf{English} $ & cell2 row 1 & cell3 row 1 & cell4 row 1 & cell5 row 1 \\ \hline
% $ \textbf{Uzbek} $ & cell2 row 2 & cell3 row 2 & cell4 row 2 & cell5 row 2  \\ \hline
% $ \textbf{Amharic} $ & cell2 row 3 & cell3 row 3 & cell4 row 3 & cell5 row 3 \\ \hline
% $ \textbf{Tamil} $ & cell2 row 1 & cell3 row 1 & cell4 row 1 & cell5 row 1 row 1\\ \hline
% $ \textbf{Arabic} $ & cell2 row 2 & cell3 row 2 & cell4 row 2 & cell5 row 2 \\ \hline
% $ \textbf{Hausa} $ & cell2 row 3 & cell3 row 3 & cell4 row 3 & cell5 row 3 \\ \hline
% \end{tabular}
% \caption{
% {\bf State-of-the-art performance reported for NER for the languages we used.}
% 'NER' results are token-level F1 scores; 'Overall' is the \ms{micro? macro?} average of the class F1 scores. 
% } % end caption
% \label{tab:neSOA}
% \end{table*}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{lrr}
% \toprule
% \textbf{Language} & \textbf{NEI-CAP} & \textbf{NEI-LM} \\ 
%  \midrule
% \textbf{English} & 83.8 & 87.2 \\ 
% \textbf{Uzbek} & 70.3 & 80.1  \\ 
% \textbf{Amharic} & - & 71.6  \\ 
% \textbf{Tamil} & - & 69.1  \\ 
% \textbf{Arabic} & - & 58.6 \\ 
% \textbf{Hausa} & 54.2 & 67.4  \\ 
% \bottomrule
% \end{tabular}
% \caption{
% NEI means Named Entity Identification, meaning finding spans only (should be high scores). NEI-CAP means identification by capitalization alone (capital tokens are tagged as entity). NEI-LM means there are two LM's, one for entity, one for non-entity. When using LM, we lowercase all text. \swm{Is this true?} Not all languages can use capitalization as a heuristic. 
% } % end caption
% \label{tab:nei}
% \end{table}


% \begin{table*}[!ht]
% \centering
% \begin{tabular}{lrrrrr}
% \toprule
% \textbf{Language} & \textbf{LM-TRAIN} & \textbf{LM-FOUND} & \textbf{CCG} & \textbf{CMU} & \textbf{SOTA} \\ 
%  \midrule
% \textbf{English}  & ? & &  & & $\sim91$ \\ 
% \textbf{Uzbek} & 57.3 & 41.3 & 75.7 & & \\ 
% \textbf{Amharic}  & 44.4  & 43.4 & 58.3 & 10.8 & \\ 
% \textbf{Tamil} & 51.6 & 20.6 &56.5 & & \\ 
% \textbf{Arabic}  & 27.9 & 21.4 & 40.2 & 50.5 & \\ 
% \textbf{Hausa} & 45.4  & 43.5 & 70.9 & 29.8 & \\ 
% \bottomrule
% \end{tabular}
% \caption{
% NER F1 scores (full labels). All datasets use PER, ORG, LOC, GPE \swm{pretty sure this isn't true...}
% } % end caption
% \label{tab:ner}
% \end{table*}

% \section{Structure}

% Language models have power to learn things in NER.
% We show that they have some power to learn on their own (and are fast)
% We show that improvements in Lample et al 2016 are largely coming from LM (maybe?)
% We show that LM added to Cogcomp NER improves
% We show that LM needs very little data to train, thus is good for low-resource tasks
% We run small-data LM on many languages, showing that it is effective.
% (All experiments will use multiple language models).

% With increasing community interest in developing Natural Language Processing (NLP) capabilities in a wide range of languages, there has been appropriate focus on ways to develop systems with minimal requirements for training data or other purpose-built human generated resources. "Chinese Room" approaches have allowed non-speakers of target languages to nevertheless annotate text in those languages to a level that supports reasonable performance on NLP tasks such as Named Entity Recognition (NER); this implies that some properties of names are inherently distinctive. Supporting evidence comes from recent development of character-level neural approaches to NER that obviate the need for comprehensive gazetteers as a key component of state-of-the-art NER systems. In this work, we investigate the discriminative power of character-level language models in identifying names vs. non-names, and in assigning types to identified names. We do this for a range of languages with the goal of assessing the potential of such models to support development of NER models for arbitrary languages. In addition, we investigate the possibility of using "found" resources such as pre-existing knowledge bases to provide the supervision needed to build these language models.  

% Research questions:
% \begin{itemize}
% \item Change in perplexity between LM for names vs. non-names
% \item If LMs are useful, how to tune parameters given zero data
% \end{itemize}

%Character-level language models (CLMs) have been used... A applies CLMs to augment the features used by their Named Entity Recognizer, observing that performance on X improves by Y on dataset Z. ...  A range of neural models operate at the character level, including \newcite{LBSKD16} work specifically on NER.  This latter work demonstrates that character-level neural model can achieve state-of-the-art performance without using gazetteers or even Brown Clusters... 

% \begin{table}
% \small
% \centering
% \begin{tabular}{lllrrr}
% \toprule
% Model & CoNLL & OntoNotes* & Enron & MASC \\
% \midrule
% Illinois & 90.51 & 76.40 & 55.89 & 59.70 \\
% CMU & 90.94 & 71.65 & 45.11 & 55.46 \\
% Stanford & && &\\
% \bottomrule
% \end{tabular}
% \caption{Phrase-level Named Entity Recognition scores for several different English datasets. This shows that adaptation is hard. Without gazetteers. Scores across domain are very bad! (* This is a cleaned version of OntoNotes, see Section ??)}
% \end{table}


% \begin{table}
% \centering
% \begin{tabular}{llrrr}
% \toprule
% Train & Test & P & R & F1 \\
% \midrule
% \multirow{4}{*}{CoNLL} & CoNLL & 91.3 & 89.6 & 90.5 \\
% & OntoNotes & 76.7 & 76.0 & 76.3 \\
% & Enron & 49.1 & 64.8 & 55.8 \\
% & MASC & 59.0 & 60.3 & 59.6 \\
% \bottomrule
% \end{tabular}
% \caption{Phrase-level Named Entity Recognition scores for several different English datasets. This shows that adaptation is hard. Without gazetteers. Scores across domain are very bad!}
% \end{table}


% \begin{table*}
% \centering
% \begin{tabular}{llrrr|r|rrr}
% \toprule
% &&&&&& \multicolumn{3}{c}{Missed}\\
% Train & Test & P & R & F1 & Unseen F1 & ORG & PER & LOC \\
% \midrule
% \multirow{4}{*}{Gigaword} & CoNLL & 94.6 & 89.8 & 92.1 &&&& \\
% & OntoNotes & 79.7 & 86.7 & 83.1 &&&& \\
% & Enron & 72.0 & 76.2 & 74.1 &&&&\\
% & MASC & 63.1 & 75.9 & 68.9 &&&& \\
% \bottomrule
% \end{tabular}
% \caption{Token level Named Entity Identification scores for several different English datasets. This model was trained on entities and non-entities from annotated gigaword.}
% \end{table*}

%\textbf{OntoNotes} Data of OntoNotes mainly comes from newswire and broadcast, which is a similar domain as CoNLL. OntoNotes has 18 labels, different from CoNLL's label sets. To better evaluate, we keep all the PER and ORG in OntoNotes, merge GPE and FAC to LOC, and replace all other labels with O. Additionally, because of the difference between the annotation guideline of CoNLL and OntoNotes, we preprocess OntoNotes data with the following rules: 1) Replace the labels of all "the" at the beginning of an entity with O. 2) Replace the labels of all "'s" at the end of a PER entity with O. 3) Do not tokenize hyphen.

%\textbf{Enron} A dataset of emails annotated only PER. To match the label set of CoNLL, we annotate ORG, LOC and MISC in Enron.

%\textbf{MASC} A mixture of data from many different domains. We keep all the PER and ORG, merge GPE to LOC, and replace all other labels with O.\\




% \subsection{Model}



%for each category of interest we use SRILM to train a CLM using tokens corresponding to that category. All tokens are converted to lowercase first. \swm{Perhaps this should be a separate experiment -- capitalization is definitely a useful feature.} For Named Entity Identification (NEI), a binary task that simply indicates whether or not a token belongs to a Named Entity, we train an in-entity CLM and a non-entity CLM. For NER, we train a CLM for each entity class and a CLM for non-entity tokens. 

%For NEI and NER, we build a token-level tagger that scans each token in the target text, lowercases it, and computes the corresponding perplexity with each CLM. It assigns the label corresponding to the CLM that assigns the lowest perplexity to that token.

% \subsection{Data}




%For the "found data" experiments, we use Wikipedia and GeoNames to identify location, organization, and person names. From GeoNames we use the alternative names field, while we use~\cite{wikipediaNer} to automatically tag target language text~\cite{someoneWhoDidThis}. For the non-entity model, we simply use monolingual text from the target language, even though $~10\%$ of tokens are expected to belong to Named Entities: our expectation is that the transition matrix learned by the CLM will have relatively low weight for in-entity transitions, if entities are markedly different from non-entities at the character sequence level (as demonstrated by the first set of experiments). 

%We will both evaluate at token-level and phrase-level. Because the CLM produces a binary decision for each token, we don't have information of the start and end index of an entity span. To evaluate at phrase-level, we simply assume that any contiguous entity tokens are part of a phrase to convert from token level (IO) to phrase level (BIO) annotations, so the first token gets a B-ENT label, and the rest are I-ENT. We make an exception in the case of social media where hashtags (\#) and handles (@) are sometimes tagged as names, and sometimes used sequentially, but nearly always are distinct phrases. For example, one might write `livin the dream \#florida \#miami \#dabeach', where `\#florida' and `\#miami' are separate entities. 

% \begin{table*}[h]
% \centering
% \begin{tabular}{lrrr|rrr}
% \toprule
% & \multicolumn{3}{c}{Token-level} & \multicolumn{3}{c}{Phrase-level} \\
% Test & P & R & F1 & P & R & F1 \\
% \midrule
% CoNLL & 94.63 & 89.879 & 92.192 & 82.48 & 81.85 & 82.16\\
% OntoNotes & 79.76 & 86.75 & 83.11 & 58.47 & 71.64 & 64.39 \\
% Enron & 72.09 & 76.23 & 74.10 & 45.93 & 58.62 & 51.51\\
% MASC & 63.09 & 75.94 & 68.92 & 46.70 & 66.61 & 54.91\\
% \bottomrule
% \end{tabular}
% \caption{Entity/non-entity language model results. Token-level and Phrase-level Named Entity Identification scores for several different English datasets. These model was trained on Entity (PER/ORG/LOC) and non-entities from annotated gigaword. OntoNotes* is again cleaned and filtered labels.}
% \end{table*}


%\textbf{NEI across domains in English }  
%Figure 1 shows that Entity CLM can confine the perplexity of most entities to a very low level, and non-entities have much higher perplexity. Though there also exists some non-entities with low perplexity, comparing the perplexity against Non-Entity CLM gives us a chance to separate entity and non-entity. Since most of entities have low perplexity, it makes sense to set a threshold that only when perplexity of Entity CLM is lower than both the threshold and the perplexity of Non-Entity CLM, we predict this token as Entity. We take threshold to be $25$ here. \xd{Need some analysis of Table 4 here}


%Table~\ref{tab:neGold} shows the results of experiments assess the potential of CLMs for Named Entity Identification and Recognition, using labeled training data from a range of languages, while table~\ref{tab:neFound} shows results using GeoNames and DBPedia in place of annotated training data. For comparison, Table~\ref{tab:neSOA} shows the performance of state-of-the-art unsupervised methods for NER on these data sets.

% \begin{table*}
% \centering
% \begin{tabular}{llrrr}
% \toprule
% Train & Test & F1-base & F1-impov & F1-impov+LM  \\
% \midrule
% \multirow{4}{*}{CoNLL} & CoNLL & 90.4 & \swm{83.0} & \swm{85.0}  \\
% & OntoNotes &  76.3 & \swm{73} & \swm{79} \\
% & Enron & 55.8 && \swm{$>55$} \\
% & MASC & 59.6 && \swm{$>60$} \\
% \bottomrule
% \end{tabular}
% \caption{Train on CoNLL, experiment with switching domains. We use an impoverished set of features when training on CoNLL, so that the CLM will learn something. \swm{Numbers in green are made up! But what we hope to see.} Scores on CoNLL go down, but scores on all other languages improve. }
% \end{table*}

%In the field of named entity recognition (NER) important features can be partitioned into token-interior features (the characters) and token-exterior features (the context of that word). While both are necessary for a high-quality NER system, we focus on the former in this work. The motivation is to improve recall by moving beyond features that fire only on exact match.  

%Lexical memorization, an extreme form of token-interior feature, is perhaps the most important, but the use of gazetteers, and token affix features point to the same thing. In practice this means that if you see a name in the past you are far more likely to predict the name in the future. 

%Naturally, this leads to problems with generalization. What can we do when we see unfamiliar tokens in unfamiliar contexts? In this work, we focus on the former problem, and leave the latter problem for future work. We believe that we can learn properties of names on training data that will generalize to unseen data. Further the properties that we will learn are based on character-level properties of words. The key observation is that names look different from other words and this difference can be learned. 

%There are two important caveats that must be made. First in the definition of the name. We focus solely on coarse-grained categories of names and avoid fine-grained definitions. Second we understand that this observation may not hold across languages, especially Semitic languages where there is little distinction between proper and common nouns. We explore this hypothesis by experimenting on a large number of languages from diverse language families. 

%Finally we show that since language models or character level features have discriminative power that these can also be used to augment standard NER systems especially to improve domain adaptation. 

%\ms{Alternatively....:}
%NER is one of the oldest established NLP task, in part because it is a lynchpin of Information Extraction. Work on NER in the last few years has followed two key paths: 1. design new features (gazetteers, brown clusters, ...?), typically adding them to the existing collection of features. While experimentally this improves performance, it also tends to increase the complexity of the model, increase memory overhead, and reduce processing speed. 2. switch to a neural approach. This sidesteps the bulk of feature engineering effort and the resulting system overhead, but has several drawbacks: training can take a long time and require expensive equipment to run; trained models are not interpretable, and their performance may be extremely variable over repeated training runs -- that is, they may overfit training data due to their inherent complexity. Both approaches, therefore, may be expected to experience problems when used to annotate new data, especially when that data is not from a domain identical to the training data. Learning theory tells us that when choosing between two models that we can expect the simpler one to be more robust: so can we identify a simpler model to use with NER
 

